Non-cyclotomic fusion categories

Etingof, Nikshych and Ostrik ask in arXiv:math.QA/0203060 if every fusion category can be completely defined over a cyclotomic field. We show that this is not the case: in particular one of the fusion categories coming from the Haagerup subfactor arXiv:math.OA/9803044 and one coming from the newly constructed extended Haagerup subfactor arXiv:0909.4099 can not be completely defined over a cyclotomic field. On the other hand, we show that the double of the even part of the Haagerup subfactor is completely defined over a cyclotomic field. We identify the minimal field of definition for each of these fusion categories, compute the Galois groups, and identify their Galois conjugates.

==> diagrams/tikz/circles.tex <==
\begin{tikzpicture}
\path (0,0) node (B') [shape=rectangle, draw]{\;$B'$\;};
\path (0,1) node (B) [shape=rectangle, draw]{\;$B$\;};

\draw [->, very thick] (B'.130) -- (B.230);
\draw [->, very thick] (B'.50) -- (B.310);
\end{tikzpicture}
